MAGIC observations provide compelling evidence of the hadronic multi-TeV emission from the putative PeVatron SNR G106.3+2.7

The SNR G106.3+2.7, detected at 1--100 TeV energies by different $\gamma$-ray facilities, is one of the most promising PeVatron candidates. This SNR has a cometary shape which can be divided into a head and a tail region with different physical conditions. However, it is not identified in which region the 100 TeV emission is produced due to the limited position accuracy and/or angular resolution of existing observational data. Additionally, it remains unclear whether the origin of the $\gamma$-ray emission is leptonic or hadronic. With the better angular resolution provided by these new MAGIC data compared to earlier $\gamma$-ray datasets, we aim to reveal the acceleration site of PeV particles and the emission mechanism by resolving the SNR G106.3+2.7 with 0.1$^\circ$ resolution at TeV energies. We detected extended $\gamma$-ray emission spatially coincident with the radio continuum emission at the head and tail of SNR G106.3+2.7. The fact that we detected a significant $\gamma$-ray emission with energies above 6.0 TeV from the tail region only suggests that the emissions above 10 TeV, detected with air shower experiments (Milagro, HAWC, Tibet AS$\gamma$ and LHAASO), are emitted only from the SNR tail. Under this assumption, the multi-wavelength spectrum of the head region can be explained with either hadronic or leptonic models, while the leptonic model for the tail region is in contradiction with the emission above 10 TeV and X-rays. In contrast, the hadronic model could reproduce the observed spectrum at the tail by assuming a proton spectrum with a cutoff energy of $\sim 1$ PeV for the tail region. Such a high energy emission in this middle-aged SNR (4--10 kyr) can be explained by considering the scenario that protons escaping from the SNR in the past interact with surrounding dense gases at present.

==> authors_last_AA.tex <==
% authors 05.04.2022  Format AA
%commento di prova file normale%
\author{
MAGIC Collaboration:
S.~Abe\inst{1} \and
H.~Abe\inst{1} \and
V.~A.~Acciari\inst{2} \and
T.~Aniello\inst{3} \and
S.~Ansoldi\inst{4,45} \and
L.~A.~Antonelli\inst{3} \and
A.~Arbet Engels\inst{5} \and
C.~Arcaro\inst{6} \and
M.~Artero\inst{7} \and
K.~Asano\inst{1} \and
D.~Baack\inst{8} \and
A.~Babi\'c\inst{9} \and
A.~Baquero\inst{10} \and
U.~Barres de Almeida\inst{11} \and
J.~A.~Barrio\inst{10} \and
I.~Batkovi\'c\inst{6} \and
J.~Baxter\inst{1} \and
J.~Becerra Gonz\'alez\inst{2} \and
W.~Bednarek\inst{12} \and
E.~Bernardini\inst{6} \and
M.~Bernardos\inst{13} \and
A.~Berti\inst{5} \and
J.~Besenrieder\inst{5} \and
W.~Bhattacharyya\inst{14} \and
C.~Bigongiari\inst{3} \and
A.~Biland\inst{15} \and
O.~Blanch\inst{7} \and
G.~Bonnoli\inst{3} \and
\v{Z}.~Bo\v{s}njak\inst{9} \and
I.~Burelli\inst{4} \and
G.~Busetto\inst{6} \and
R.~Carosi\inst{16} \and
M.~Carretero-Castrillo\inst{17} \and
G.~Ceribella\inst{1} \and
Y.~Chai\inst{5} \and
A.~Chilingarian\inst{18} \and
S.~Cikota\inst{9} \and
E.~Colombo\inst{2} \and
J.~L.~Contreras\inst{10} \and
J.~Cortina\inst{19} \and
S.~Covino\inst{3} \and
G.~D'Amico\inst{20} \and
V.~D'Elia\inst{3} \and
P.~Da Vela\inst{16,46} \and
F.~Dazzi\inst{3} \and
A.~De Angelis\inst{6} \and
B.~De Lotto\inst{4} \and
A.~Del Popolo\inst{21} \and
M.~Delfino\inst{7,47} \and
J.~Delgado\inst{7,47} \and
C.~Delgado Mendez\inst{19} \and
D.~Depaoli\inst{22} \and
F.~Di Pierro\inst{22} \and
L.~Di Venere\inst{23} \and
E.~Do Souto Espi\~neira\inst{7} \and
D.~Dominis Prester\inst{24} \and
A.~Donini\inst{3} \and
D.~Dorner\inst{25} \and
M.~Doro\inst{6} \and
D.~Elsaesser\inst{8} \and
G.~Emery\inst{26} \and
V.~Fallah Ramazani\inst{27,48} \and
L.~Fari\~na\inst{7} \and
A.~Fattorini\inst{8} \and
L.~Font\inst{28} \and
C.~Fruck\inst{5} \and
S.~Fukami\inst{15} \and
Y.~Fukazawa\inst{29} \and
R.~J.~Garc\'ia L\'opez\inst{2} \and
M.~Garczarczyk\inst{14} \and
S.~Gasparyan\inst{30} \and
M.~Gaug\inst{28} \and
J.~G.~Giesbrecht Paiva\inst{11} \and
N.~Giglietto\inst{23} \and
F.~Giordano\inst{23} \and
P.~Gliwny\inst{12} \and
N.~Godinovi\'c\inst{31} \and
J.~G.~Green\inst{5} \and
D.~Green\inst{5} \and
D.~Hadasch\inst{1} \and
A.~Hahn\inst{5} \and
T.~Hassan\inst{19} \and
L.~Heckmann\inst{5,49} \and
J.~Herrera\inst{2} \and
D.~Hrupec\inst{32} \and
M.~H\"utten\inst{1} \and
R.~Imazawa\inst{29} \and
T.~Inada\inst{1} \and
R.~Iotov\inst{25} \and
K.~Ishio\inst{12} \and
I.~Jim\'enez Mart\'inez\inst{19} \and
J.~Jormanainen\inst{27} \and
D.~Kerszberg\inst{7} \and
Y.~Kobayashi\inst{1} \and
H.~Kubo\inst{1} \and
J.~Kushida\inst{33} \and
A.~Lamastra\inst{3} \and
D.~Lelas\inst{31} \and
F.~Leone\inst{3} \and
E.~Lindfors\inst{27} \and
L.~Linhoff\inst{8} \and
S.~Lombardi\inst{3} \and
F.~Longo\inst{4,50} \and
R.~L\'opez-Coto\inst{6} \and
M.~L\'opez-Moya\inst{10} \and
A.~L\'opez-Oramas\inst{2} \and
S.~Loporchio\inst{23} \and
A.~Lorini\inst{34} \and
E.~Lyard\inst{26} \and
B.~Machado de Oliveira Fraga\inst{11} \and
P.~Majumdar\inst{35,51} \and
M.~Makariev\inst{36} \and
G.~Maneva\inst{36} \and
N.~Mang\inst{8} \and
M.~Manganaro\inst{24} \and
S.~Mangano\inst{19} \and
K.~Mannheim\inst{25} \and
M.~Mariotti\inst{6} \and
M.~Mart\'inez\inst{7} \and
A.~Mas Aguilar\inst{10} \and
D.~Mazin\inst{1,52} \and
S.~Menchiari\inst{34} \and
S.~Mender\inst{8} \and
S.~Mi\'canovi\'c\inst{24} \and
D.~Miceli\inst{6} \and
T.~Miener\inst{10} \and
J.~M.~Miranda\inst{34} \and
R.~Mirzoyan\inst{5} \and
E.~Molina\inst{17} \and
H.~A.~Mondal\inst{35} \and
A.~Moralejo\inst{7} \and
D.~Morcuende\inst{10} \and
V.~Moreno\inst{28} \and
T.~Nakamori\inst{37} \and
C.~Nanci\inst{3} \and
L.~Nava\inst{3} \and
V.~Neustroev\inst{38} \and
M.~Nievas Rosillo\inst{2} \and
C.~Nigro\inst{7} \and
K.~Nilsson\inst{27} \and
K.~Nishijima\inst{33} \and
T.~Njoh Ekoume\inst{2} \and
K.~Noda\inst{1} \and
S.~Nozaki\inst{5} \and
Y.~Ohtani\inst{1} \and
T.~Oka\inst{39} \and
J.~Otero-Santos\inst{2} \and
S.~Paiano\inst{3} \and
M.~Palatiello\inst{4} \and
D.~Paneque\inst{5} \and
R.~Paoletti\inst{34} \and
J.~M.~Paredes\inst{17} \and
L.~Pavleti\'c\inst{24} \and
M.~Persic\inst{4,53} \and
M.~Pihet\inst{5} \and
F.~Podobnik\inst{34} \and
P.~G.~Prada Moroni\inst{16} \and
E.~Prandini\inst{6} \and
G.~Principe\inst{4} \and
C.~Priyadarshi\inst{7} \and
I.~Puljak\inst{31} \and
W.~Rhode\inst{8} \and
M.~Rib\'o\inst{17} \and
J.~Rico\inst{7} \and
C.~Righi\inst{3} \and
A.~Rugliancich\inst{16} \and
N.~Sahakyan\inst{30} \and
T.~Saito\inst{1} \and
S.~Sakurai\inst{1} \and
K.~Satalecka\inst{27} \and
F.~G.~Saturni\inst{3} \and
B.~Schleicher\inst{25} \and
K.~Schmidt\inst{8} \and
F.~Schmuckermaier\inst{5} \and
J.~L.~Schubert\inst{8} \and
T.~Schweizer\inst{5} \and
J.~Sitarek\inst{12} \and
V.~Sliusar\inst{26} \and
D.~Sobczynska\inst{12} \and
A.~Spolon\inst{6} \and
A.~Stamerra\inst{3} \and
J.~Stri\v{s}kovi\'c\inst{32} \and
D.~Strom\inst{5} \and
M.~Strzys\inst{1} \and
Y.~Suda\inst{29} \and
T.~Suri\'c\inst{40} \and
M.~Takahashi\inst{41} \and
R.~Takeishi\inst{1} \and
F.~Tavecchio\inst{3} \and
P.~Temnikov\inst{36} \and
K.~Terauchi\inst{39} \and
T.~Terzi\'c\inst{24} \and
M.~Teshima\inst{5,54} \and
L.~Tosti\inst{42} \and
S.~Truzzi\inst{34} \and
A.~Tutone\inst{3} \and
S.~Ubach\inst{28} \and
J.~van Scherpenberg\inst{5} \and
M.~Vazquez Acosta\inst{2} \and
S.~Ventura\inst{34} \and
V.~Verguilov\inst{36} \and
I.~Viale\inst{6} \and
C.~F.~Vigorito\inst{22} \and
V.~Vitale\inst{43} \and
I.~Vovk\inst{1} \and
R.~Walter\inst{26} \and
M.~Will\inst{5} \and
C.~Wunderlich\inst{34} \and
T.~Yamamoto\inst{44} \and
D.~Zari\'c\inst{31}
}
\institute { Japanese MAGIC Group: Institute for Cosmic Ray Research (ICRR), The University of Tokyo, Kashiwa, 277-8582 Chiba, Japan
\and Instituto de Astrof\'isica de Canarias and Dpto. de  Astrof\'isica, Universidad de La Laguna, E-38200, La Laguna, Tenerife, Spain
\and National Institute for Astrophysics (INAF), I-00136 Rome, Italy
\and Universit\`a di Udine and INFN Trieste, I-33100 Udine, Italy
\and Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany
\and Universit\`a di Padova and INFN, I-35131 Padova, Italy
\and Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain
\and Technische Universit\"at Dortmund, D-44221 Dortmund, Germany
\and Croatian MAGIC Group: University of Zagreb, Faculty of Electrical Engineering and Computing (FER), 10000 Zagreb, Croatia
\and IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain
\and Centro Brasileiro de Pesquisas F\'isicas (CBPF), 22290-180 URCA, Rio de Janeiro (RJ), Brazil
\and University of Lodz, Faculty of Physics and Applied Informatics, Department of Astrophysics, 90-236 Lodz, Poland
\and Instituto de Astrof\'isica de Andaluc\'ia-CSIC, Glorieta de la Astronom\'ia s/n, 18008, Granada, Spain
\and Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany
\and ETH Z\"urich, CH-8093 Z\"urich, Switzerland
\and Universit\`a di Pisa and INFN Pisa, I-56126 Pisa, Italy
\and Universitat de Barcelona, ICCUB, IEEC-UB, E-08028 Barcelona, Spain
\and Armenian MAGIC Group: A. Alikhanyan National Science Laboratory, 0036 Yerevan, Armenia
\and Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas, E-28040 Madrid, Spain
\and Department for Physics and Technology, University of Bergen, Norway
\and INFN MAGIC Group: INFN Sezione di Catania and Dipartimento di Fisica e Astronomia, University of Catania, I-95123 Catania, Italy
\and INFN MAGIC Group: INFN Sezione di Torino and Universit\`a degli Studi di Torino, I-10125 Torino, Italy
\and INFN MAGIC Group: INFN Sezione di Bari and Dipartimento Interateneo di Fisica dell'Universit\`a e del Politecnico di Bari, I-70125 Bari, Italy
\and Croatian MAGIC Group: University of Rijeka, Department of Physics, 51000 Rijeka, Croatia
\and Universit\"at W\"urzburg, D-97074 W\"urzburg, Germany
\and University of Geneva, Chemin d'Ecogia 16, CH-1290 Versoix, Switzerland
\and Finnish MAGIC Group: Finnish Centre for Astronomy with ESO, University of Turku, FI-20014 Turku, Finland
\and Departament de F\'isica, and CERES-IEEC, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Spain
\and Japanese MAGIC Group: Physics Program, Graduate School of Advanced Science and Engineering, Hiroshima University, 739-8526 Hiroshima, Japan
\and Armenian MAGIC Group: ICRANet-Armenia at NAS RA, 0019 Yerevan, Armenia
\and Croatian MAGIC Group: University of Split, Faculty of Electrical Engineering, Mechanical Engineering and Naval Architecture (FESB), 21000 Split, Croatia
\and Croatian MAGIC Group: Josip Juraj Strossmayer University of Osijek, Department of Physics, 31000 Osijek, Croatia
\and Japanese MAGIC Group: Department of Physics, Tokai University, Hiratsuka, 259-1292 Kanagawa, Japan
\and Universit\`a di Siena and INFN Pisa, I-53100 Siena, Italy
\and Saha Institute of Nuclear Physics, A CI of Homi Bhabha National Institute, Kolkata 700064, West Bengal, India
\and Inst. for Nucl. Research and Nucl. Energy, Bulgarian Academy of Sciences, BG-1784 Sofia, Bulgaria
\and Japanese MAGIC Group: Department of Physics, Yamagata University, Yamagata 990-8560, Japan
\and Finnish MAGIC Group: Space Physics and Astronomy Research Unit, University of Oulu, FI-90014 Oulu, Finland
\and Japanese MAGIC Group: Department of Physics, Kyoto University, 606-8502 Kyoto, Japan
\and Croatian MAGIC Group: Ru\dj{}er Bo\v{s}kovi\'c Institute, 10000 Zagreb, Croatia
\and Japanese MAGIC Group: Institute for Space-Earth Environmental Research and Kobayashi-Maskawa Institute for the Origin of Particles and the Universe, Nagoya University, 464-6801 Nagoya, Japan
\and INFN MAGIC Group: INFN Sezione di Perugia, I-06123 Perugia, Italy
\and INFN MAGIC Group: INFN Roma Tor Vergata, I-00133 Roma, Italy
\and Japanese MAGIC Group: Department of Physics, Konan University, Kobe, Hyogo 658-8501, Japan
\and also at International Center for Relativistic Astrophysics (ICRA), Rome, Italy
\and now at University of Innsbruck, Institute for Astro and Particle Physics
\and also at Port d'Informaci\'o Cient\'ifica (PIC), E-08193 Bellaterra (Barcelona), Spain
\and now at Ruhr-Universit\"at Bochum, Fakult\"at f\"ur Physik und Astronomie, Astronomisches Institut (AIRUB), 44801 Bochum, Germany
\and also at University of Innsbruck, Institute for Astro- and Particle Physics
\and also at Dipartimento di Fisica, Universit\`a di Trieste, I-34127 Trieste, Italy
\and also at University of Lodz, Faculty of Physics and Applied Informatics, Department of Astrophysics, 90-236 Lodz, Poland
\and Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany
\and also at INAF Trieste and Dept. of Physics and Astronomy, University of Bologna, Bologna, Italy
\and Japanese MAGIC Group: Institute for Cosmic Ray Research (ICRR), The University of Tokyo, Kashiwa, 277-8582 Chiba, Japan
}

